SEAL: A Framework for Systematic Evaluation of Real-World Super-Resolution

Real-world Super-Resolution (Real-SR) methods focus on dealing with diverse real-world images and have attracted increasing attention in recent years. The key idea is to use a complex and high-order degradation model to mimic real-world degradations. Although they have achieved impressive results in various scenarios, they are faced with the obstacle of evaluation. Currently, these methods are only assessed by their average performance on a small set of degradation cases randomly selected from a large space, which fails to provide a comprehensive understanding of their overall performance and often yields inconsistent and potentially misleading results. To overcome the limitation in evaluation, we propose SEAL, a framework for systematic evaluation of real-SR. In particular, we cluster the extensive degradation space to create a set of representative degradation cases, which serves as a comprehensive test set. Next, we propose a coarse-to-fine evaluation protocol to measure the distributed and relative performance of real-SR methods on the test set. The protocol incorporates two new metrics: acceptance rate (AR) and relative performance ratio (RPR), derived from acceptance and excellence lines. Under SEAL, we benchmark existing real-SR methods, obtain new observations and insights into their performance, and develop a new strong baseline. We consider SEAL as the first step towards creating a comprehensive real-SR evaluation platform, which can promote the development of real-SR. The source code is available at https://github.com/XPixelGroup/SEAL

==> Table1.tex <==

\begin{table}[t]
\caption{Quantitative results of different methods on DIV2K5G. Group0 denotes the validation set with satisfactory degradation tasks, and Group1-4 represent the validation sets with unsatisfactory degradation tasks. The top two results are marked in \textcolor{red}{red} and \textcolor{blue}{blue}, respectively. The ESRGAN trained on the non-blind setting and RDSR trained on the MSE-based setting are marked in \textcolor{gray}{gray}.}
\label{tab_results1}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lcccccccccc} \toprule
 & \multicolumn{2}{c}{Group0} & \multicolumn{2}{c}{Group1} & \multicolumn{2}{c}{Group2} & \multicolumn{2}{c}{Group3} & \multicolumn{2}{c}{Group4} \\ 
               & PSNR  & LPIPS  & PSNR  & LPIPS  & PSNR  & LPIPS  & PSNR  & LPIPS  & PSNR  & LPIPS  \\ \midrule
\textcolor{gray}{ESRGAN}         & \textcolor{gray}{21.49} & \textcolor{gray}{0.6166} & \textcolor{gray}{20.29} & \textcolor{gray}{0.6697} & \textcolor{gray}{20.95} & \textcolor{gray}{0.6530} & \textcolor{gray}{22.42} & \textcolor{gray}{0.5940}  & \textcolor{gray}{22.02} & \textcolor{gray}{0.5837} \\
\textcolor{gray}{RDSR}           & \textcolor{gray}{25.00} & \textcolor{gray}{0.5196} & \textcolor{gray}{21.18} & \textcolor{gray}{0.6167} & \textcolor{gray}{23.06} & \textcolor{gray}{0.5586} & \textcolor{gray}{25.00} & \textcolor{gray}{0.4993} & \textcolor{gray}{25.58} & \textcolor{gray}{0.4814} \\
MM-RealSR      & 23.49 & 0.4549 & 19.74 & 0.5326 & 21.76 & 0.4731 & 23.37 & 0.4205 & 23.97 & 0.3989 \\
DASR           & 23.87 & 0.4683 & 19.97 & 0.5752 & 22.31 & 0.5093 & 24.00 & 0.4474 & 24.85 & 0.4225 \\
BSRGAN         & 23.99 & 0.4549 & 20.07 & 0.5799 & 22.45 & 0.4961 & 24.34 & 0.4388 & 24.80 & 0.4210  \\ \midrule
% Real-ESRGAN    & 23.85 & 0.4325 & 20.10 & 0.5355 & 22.07 & 0.4701 & 24.30 & 0.4147 & 24.58 & 0.3970  \\ 
Real-SRGAN     & 23.88 & 0.4599 & 20.10 & 0.5586 & 22.12 & 0.5019 & 23.85 & 0.4499 & 24.48 & 0.4270         \\
Real-SRGAN-TG  & 23.95 & 0.4617 & 21.14 & 0.5323 & 23.06 & 0.4802 &  24.69& 0.4248 & 25.05 & 0.4112 \\ \midrule
Real-ESRGAN    & 23.85 & 0.4325 & 20.10 & 0.5355 & 22.07 & 0.4701 & 24.30 & 0.4147 & 24.58 & 0.3970  \\
Real-ESRGAN-TG & 23.99 & 0.4286 & 21.10 & 0.5056 & 23.15 & 0.4494 & 24.62 & 0.3975 & 25.03 & 0.3851 \\ \midrule
Real-SwinIR         & 23.35 & 0.4468 & 19.60 & 0.5624 & 21.65 & 0.4905 & 23.66 & 0.4265 & 24.16 & 0.4077 \\
Real-SwinIR-TG & 23.90 & 0.4168 & 20.62 & 0.4925 & 22.70 & 0.4377 & 24.56 & 0.3815 & 24.98 & 0.3670  \\ \midrule
Real-HAT       & 24.26 & 0.4084 & 20.64 & 0.5022 & 22.44 & 0.4468 & 24.42 & 0.3918 & 25.02 & 0.3734 \\
Real-HAT-TG    & 24.31 & 0.4110 & 21.41 & 0.4932 & 23.20 & 0.4395 & 24.87 & 0.3841 & 25.32 & 0.3674  \\ \bottomrule
\end{tabular}
}
\end{table}


\begin{table}[h]
\centering
\caption{Quantitative results of different methods on DIV2K5G. Group0 denotes the validation set with satisfactory degradation tasks, and Group1-4 represent the validation sets with unsatisfactory degradation tasks. The top two results are marked in \textcolor{red}{red} and \textcolor{blue}{blue}, respectively. The ESRGAN trained on the non-blind setting and RDSR trained on the MSE-based setting are marked in \textcolor{gray}{gray}.}
\label{tab:my-table}
\resizebox{0.9\textwidth}{!}{%
\begin{tabular}{lcccccccccc} \toprule
              & \multicolumn{2}{c}{DIV2K\_random} & \multicolumn{2}{c}{AIM2019} & \multicolumn{2}{c}{RealSRset-Nikon} & \multicolumn{2}{c}{RealSRset-Cano} \\
               & PSNR        & LPIPS  & PSNR    & LPIPS  & PSNR            & LPIPS  & PSNR           & LPIPS  \\ \midrule
\textcolor{gray}{ESRGAN}         & \textcolor{gray}{20.63}       & \textcolor{gray}{0.6345} & \textcolor{gray}{23.16}   & \textcolor{gray}{0.5500}   & \textcolor{gray}{27.40}        & \textcolor{gray}{0.4132} & \textcolor{gray}{27.73}          & \textcolor{gray}{0.4054} \\
\textcolor{gray}{RDSR}           & \textcolor{gray}{24.61}       & \textcolor{gray}{0.5268} & \textcolor{gray}{24.44}   & \textcolor{gray}{0.4803} & \textcolor{gray}{26.39}           & \textcolor{gray}{0.4053} & \textcolor{gray}{26.93}          & \textcolor{gray}{0.3795}        \\
MM-RealSR      & 23.17       & 0.4394 & 23.48   & 0.3917   & 23.78        & 0.3841       & 24.42    & 0.3664       \\
DASR           & 23.52       & 0.4832 & 23.76   & 0.4210  & 26.68           & 0.3972 & 27.68          & 0.3792 \\
BSRGAN         & 23.76       & 0.4622 & 24.20   & 0.4000  & 26.11           & 0.3900   & 26.90           & 0.3648 \\ 
SwinIR         & 23.13       & 0.4432 & 23.89   & 0.3870  & 26.20            & 0.3616 & 26.68          & 0.3469 \\
Real-ESRGAN     & 23.54       & 0.4423 & 23.89   & 0.3960  & 25.62           & 0.3820  & 26.06          & 0.3629 \\

\midrule
Real-SRGAN     & 23.58 &0.4710 & 23.72 & 0.4247 & 24.71  & 0.4159 & 25.42  & 0.3902  \\
Real-SRGAN-TG  & 23.79 &0.4705 & 23.97 & 0.4174 & 25.18  & 0.4018 & 25.93  & 0.3759 \\\midrule
Real-ESRGAN     & 23.54       & 0.4423 & 23.89   & 0.3960  & 25.62         & 0.3820  & 26.06          & 0.3629 \\
Real-ESRGAN-TG  & 23.84       & 0.4368 & 24.27   & 0.3899 & 26.01           & 0.3819 & 26.33          & 0.3637 \\\midrule
Real-SwinIR    & 23.67       & 0.4216 & 23.98   & 0.3804 & 25.70            & 0.3700   & 26.43          & 0.3506 \\
Real-SwinIR-TG & 23.74       & 0.4190  & 24.10  & 0.3766 & 26.36           & 0.3751 & 27.18          & 0.3585 \\\midrule
Real-HAT       & 24.04       & 0.4156 & 24.19   & 0.3742 & 25.88           & 0.3532 & 26.56          & 0.3339 \\
Real-HAT-TG    & 24.21       & 0.4189 & 24.41   & 0.3723 & 26.12           & 0.3635 & 26.69          & 0.3451 \\ \bottomrule
\end{tabular}
}
\end{table}


==> Table2.tex <==
\begin{table*}[t]
\renewcommand\arraystretch{1.0}
\caption{Classification accuracy on CIFAR-100 for 5-way 5-shot incremental learning. \textsuperscript{$\ast$} indicates our re-implementation.} 
\label{tab_cifar}
\centering
\resizebox{0.9\textwidth}{!}{
\begin{tabular}{lcccccccccc}
  \toprule
  \multirow[m]{2}{*}{\textbf{Method}} & \multicolumn{9}{c}{\textbf{sessions}} & \multirow[m]{2}{*}{\shortstack{\textbf{The gap}\\ \textbf{with cRT}}}\\
  \cmidrule[0.05em]{2-10}
  & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 &\\
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5
  \midrule
  cRT~\cite{cRT}\textsuperscript{$\ast$}            & 65.18 & 63.89 & 60.20 & 57.23 & 53.71 & 50.39 & 48.77 & 47.29 & 45.28 & -\\
  Joint-training\textsuperscript{$\ast$}               & 65.18 & 61.45 & 57.36 & 53.68 & 50.84 & 47.33 & 44.79 & 42.62 & 40.08 & -5.20\\
  Baseline                                          & 65.18 & 61.67 & 58.61 & 55.11 & 51.86 & 49.43 & 47.60 & 45.64 & 43.83 & -1.45\\
  \midrule
  iCaRL~\cite{icarl}\textsuperscript{$\ast$}        & 66.52 & 57.26 & 54.27 & 50.62 & 47.33 & 44.99 & 43.14 & 41.16 & 39.49 & -5.79\\
  Rebalance~\cite{NCM}\textsuperscript{$\ast$}      & \textbf{66.66} & 61.42 & 57.29 & 53.02 & 48.85 & 45.68 & 43.06 & 40.56 & 38.35 & -6.93 \\
  FSLL~\cite{FSLL}\textsuperscript{$\ast$}          & 65.18 & 56.24 & 54.55 & 51.61 & 49.11 & 47.27 & 45.35 & 43.95 & 42.22 & -3.08\\
  iCaRL~\cite{icarl}     & 64.10 & 53.28 & 41.69 & 34.13 & 27.93 & 25.06 & 20.41 & 15.48 & 13.73 & -31.55\\
  Rebalance~\cite{NCM}   & 64.10 & 53.05 & 43.96 & 36.97 & 31.61 & 26.73 & 21.23 & 16.78 & 13.54 & -31.74\\
  %ProtoNet~\cite{PN}     & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & \\
  TOPIC~\cite{TOPIC}     & 64.10 & 55.88 & 47.07 & 45.16 & 40.11 & 36.38 & 33.96 & 31.55 & 29.37 & -15.91 \\
  FSLL~\cite{FSLL}       & 64.10 & 55.85 & 51.71 & 48.59 & 45.34 & 43.25 & 41.52 & 39.81 & 38.16 & -7.12\\
  FSLL+SS~\cite{FSLL}    & 66.76 & 55.52 & 52.20 & 49.17 & 46.23 & 44.64 & 43.07 & 41.20 & 39.57 & -5.71\\
  \midrule
  \textbf{F2M}                   & 64.71 & \textbf{62.05} & \textbf{59.01} & \textbf{55.58} & \textbf{52.55} & \textbf{49.96} & \textbf{48.08} & \textbf{46.28} & \textbf{44.67} & \textbf{-0.61}\\
  \bottomrule
\end{tabular}
}
\end{table*}


==> Table3.tex <==
\begin{table*}[t]
\renewcommand\arraystretch{1.0}
\caption{Classification accuracy on CUB-200-2011 for 10-way 5-shot incremental learning.\textsuperscript{$\ast$} indicates our re-implementation.} 
\label{tab_cub}
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{lcccccccccccc}
  \toprule
  \multirow[m]{2}{*}{\textbf{Method}} & \multicolumn{11}{c}{\textbf{sessions}} & \multirow[m]{2}{*}{\shortstack{\textbf{The gap}\\ \textbf{with cRT}}}\\
  \cmidrule[0.05em]{2-12}
  & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11\\
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5
  \midrule
  cRT~\cite{cRT}\textsuperscript{$\ast$}      & 80.83 & 78.51 & 76.12 & 73.93 & 71.46 & 68.96 & 67.73 & 66.75 & 64.22 & 62.53 & 61.08 & -\\
  Joint-training\textsuperscript{$\ast$}         & 80.83 & 77.57 & 74.11 & 70.75 & 68.52 & 65.97 & 64.58 & 62.22 & 60.18 & 58.49 & 56.78 & -4.30 \\
  Baseline                                    & 80.87 & 77.15 & 74.46 & 72.26 & 69.47 & 67.18 & 65.62 & 63.68 & 61.30 & 59.72 & 58.12 & -2.96\\
  \midrule
  iCaRL~\cite{icarl}\textsuperscript{$\ast$}  & 79.58 & 67.63 & 64.17 & 61.80 & 58.10 & 55.51 & 53.34 & 50.89 & 48.62 & 47.34 & 45.60 & -15.48\\
  Rebalance~\cite{NCM}\textsuperscript{$\ast$}& 80.94 & 70.32 & 62.96 & 57.19 & 51.06 & 46.70 & 44.03 & 40.15 & 36.75 & 34.88 & 32.09 & -28.99\\
  FSLL~\cite{FSLL}\textsuperscript{$\ast$}    & 80.83 & 77.38 & 72.37 & 71.84 & 67.51 & 65.30 & 63.75 & 61.16 & 59.05 & 58.03 & 55.82 & -5.26\\
  iCaRL~\cite{icarl}     & 68.68 & 52.65 & 48.61 & 44.16 & 36.62 & 29.52 & 27.83 & 26.26 & 24.01 & 23.89 & 21.16 & -39.92\\
  Rebalance~\cite{NCM}   & 68.68 & 57.12 & 44.21 & 28.78 & 26.71 & 25.66 & 24.62 & 21.52 & 20.12 & 20.06 & 19.87 & -41.21\\
  %ProtoNet~\cite{PN}     & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 \\
  TOPIC~\cite{TOPIC}     & 68.68 & 62.49 & 54.81 & 49.99 & 45.25 & 41.40 & 38.35 & 35.36 & 32.22 & 28.31 & 26.28 & -34.80\\
  FSLL~\cite{FSLL}       & 72.77 & 69.33 & 65.51 & 62.66 & 61.10 & 58.65 & 57.78 & 57.26 & 55.59 & 55.39 & 54.21 & -6.87\\
  FSLL+SS~\cite{FSLL}    & 75.63 & 71.81 & 68.16 & 64.32 & 62.61 & 60.10 & 58.82 & 58.70 & 56.45 & 56.41 & 55.82 & -5.26\\
  IDLVQ-C~\cite{IDLVQC}  & 77.37 & 74.72 & 70.28 & 67.13 & 65.34 & 63.52 & 62.10 & 61.54 & 59.04 & 58.68 & 57.81 & -3.27\\
  \midrule
  \textbf{F2M}                    & \textbf{81.07} & \textbf{78.16} & \textbf{75.57} & \textbf{72.89} & \textbf{70.86} & \textbf{68.17} & \textbf{67.01} & \textbf{65.26} & \textbf{63.36} & \textbf{61.76} & \textbf{60.26} & \textbf{-0.82}\\
  \bottomrule
\end{tabular}
}
\end{table*}



==> Table4.tex <==
\begin{table*}[t]
\renewcommand\arraystretch{1.0}
\caption{Ablation study on CIFAR-100 to analyze the effectiveness of different designs in F2M. \textbf{PD} refers to the performance dropping rate.} 
\label{table:ablation}
\centering
\resizebox{0.92\textwidth}{!}{
\begin{tabular}{cccccccccccccc}
  \toprule
  \multirow[m]{2}{*}{\textbf{FM}} & \multirow[m]{2}{*}{\textbf{PF}} & \multirow[m]{2}{*}{\textbf{PC}} & \multirow[m]{2}{*}{\textbf{Normalize}} & \multicolumn{9}{c}{\textbf{sessions}} & \multirow[m]{2}{*}{\textbf{PD}\downarrow}\\
  \cmidrule[0.05em]{5-13}
  & & & & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & \\
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5
  \midrule
                &            &            &            & \textbf{65.18} & 60.83 & 53.13 & 43.57 & 23.75 & 10.76 & 08.26 & 07.24 & 06.45 & 58.73\\
                &            & \checkmark &            & \textbf{65.18} & 59.48 & 56.77 & 52.99 & 50.09 & 47.80 & 45.92 & 44.20 & 42.55 & 22.63\\    
     \checkmark & \checkmark &            & \checkmark & 64.71 & 59.54 & 53.03 & 45.09 & 41.68 & 39.04 & 38.64 & 37.19 & 36.01 & 28.70 \\
     \checkmark &            & \checkmark & \checkmark & 64.55 & 61.27 & 58.33 & 54.82 & 51.60 & 49.22 & 47.48 & 45.78 & 44.08 & 20.47\\
     \checkmark & \checkmark & \checkmark &            & 64.71 & 61.75 & 58.80 & 55.33 & 52.27 & 49.75 & 47.72 & 46.01 & 44.43 & 20.28\\
  % Without Normlization   & 65.18 & 61.67 & 58.61 & 55.11 & 51.86 & 49.43 & 47.60 & 45.64 & 43.83 \\
  \midrule
     \checkmark & \checkmark & \checkmark & \checkmark & 64.71 & \textbf{61.99} & \textbf{58.99} & \textbf{55.58} & \textbf{52.55} & \textbf{49.96} & \textbf{48.08} & \textbf{46.28} & \textbf{44.67} & \textbf{20.04}\\
  \bottomrule
\end{tabular}
}
\end{table*}


%   \midrule
%   Baseline                                  & & & 65.18 & 61.67 & 58.61 & 55.11 & 51.86 & 49.43 & 47.60 & 45.64 & 43.83 \\
%   $\mathcal{L}_{ce}$ + Tuning whole model   & & & 65.18 & 60.83 & 53.13 & 43.57 & 23.75 & 10.76 & 08.26 & 07.24 & 06.45 \\
%   $\mathcal{L}_{ce}$ + Tuning BN + Clamping & & & 65.18 & 59.48 & 56.77 & 52.99 & 50.09 & 47.80 & 45.92 & 44.20 & 42.55 \\
%   Flat Minima + w/o Normalization           & & & 65.18 & 61.67 & 58.61 & 55.11 & 51.86 & 49.43 & 47.60 & 45.64 & 43.83 \\
%   % Without Normlization   & 65.18 & 61.67 & 58.61 & 55.11 & 51.86 & 49.43 & 47.60 & 45.64 & 43.83 \\
%   \midrule
%   FFM                                       & & & 64.71 & 61.99 & 58.99 & 55.58 & 52.55 & 49.96 & 48.08 & 46.28 & 44.67 \\
%   \bottomrule

==> Table5.tex <==
\begin{table*}[t]
\renewcommand\arraystretch{1.0}
\caption{The cross domain setting. miniImaget->CUB} 
\label{tab_cub}
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{lcccc}
  \toprule
  \multirow[m]{2}{*}{\textbf{Method}} & \multicolumn{11}{c}{\textbf{sessions}}\\
  \cmidrule[0.05em]{2-12}
  & 1 & 2 & 3 & 4 \\
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5
  \midrule
  Joint-train            & 65.18 & 61.45 & 57.36 & 53.68 & 50.84 & 47.33 & 44.79 & 42.62 & 40.08 & 00.00 & 00.00\\
  cRT~\cite{cRT}         & 65.18 & 61.45 & 57.36 & 57.32 & 54.22 & 51.13 & 48.44 & 46.62 & 44.60 & 00.00 & 00.00\\
  Baseline               & 79.10 & 68.69 & 58.40 & 48.12 & 53.28 & 50.50 & 47.96 & 45.85 & 43.88 & 00.00 & 00.00\\
  \midrule
  iCaRL~\cite{icarl}     & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 \\
  NCM~\cite{NCM}         & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 \\
  %ProtoNet~\cite{PN}     & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 \\
  TOPIC~\cite{TOPIC}     & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 \\
  FSLL~\cite{FSLL}       & 72.77 & 69.33 & 65.51 & 62.66 & 61.10 & 58.65 & 57.78 & 57.26 & 55.59 & 55.39 & 54.21 \\
  FSLL+SS~\cite{FSLL}    & 75.63 & 71.81 & 68.16 & 64.32 & 62.61 & 60.10 & 58.82 & 58.70 & 56.45 & 56.41 & 55.82 \\
  IDLVQ-C~\cite{IDLVQC}  & 77.37 & 74.72 & 70.28 & 67.13 & 65.34 & 63.52 & 62.10 & 61.54 & 59.04 & 58.68 & 57.81 \\
  \midrule
  Ours        & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 \\
  \bottomrule
\end{tabular}
}
\end{table*}



==> intro.tex <==
\section{Introduction}

Image super-resolution (SR) aims to reconstruct high-resolution (HR) images from their low-resolution (LR) counterparts. Recent years have witnessed great success in classical SR settings (i.e., bicubic downsampling) with deep learning techniques~\cite{dong2014learning, zhang2018rcan, zhang2018residual, ledig2017photo, Wang2018ESRGAN}. To further approach real-world applications, a series of ``blind'' SR methods have been proposed to deal with complex and unknown degradation kernels~\cite{zhang2018learning,gu2019blind,wang2021unsupervised,luo2020unfolding}. Among them, real-SR methods, such as BSRGAN~\cite{zhang2021designing} and RealESRGAN~\cite{wang2021real}, have attracted increasing attention due to their impressive results in various real-world scenarios.
Different from classical SR that only adopts a simple downsampling kernel, real-SR methods propose complex degradation models (e.g., a sequence of blurring, resizing and compression operations) that can represent a much larger degradation space, covering a wide range of real-world cases. 
However, they also face an essential \textit{dilemma}: 

\textit{Is it sufficient or complete to evaluate the real-SR model from a vast degradation space using existing evaluation approach?}



\begin{figure}[t]
\centering


\begin{subfigure}{0.4\textwidth}
\includegraphics[width=1\textwidth]{Figures/bsresr_point4.pdf}
\caption{Results under the conventional evaluation method.}
\label{fig: conventional performance}
\end{subfigure} \hspace{0.5cm}
\begin{subfigure}{0.4\textwidth}
  \includegraphics[width=1\textwidth]{Figures/bsr_esr_intro2.pdf}
  \caption{
  %Distributed performance of our proposed evaluation
  Results under our proposed evaluation framework.}
\label{fig: distributed performance}
\end{subfigure}

  \caption{(a) We follow common practice to randomly sample 2 test sets and compare the average performance of BSRNet and RealESRNet on each set. There is a significant variance in their performance: the differences in PSNR are -0.23dB and 0.18dB for BSRNet and RealESRNet respectively, leading to contradictory conclusions about their performance.
  %The observed PSNR differences are biased and opposite: 0.18dB and -0.23dB. 
  (b) BSRNet and RealESRNet assessed under our proposed evaluation framework in a distributed manner with 100 representative test sets. It shows the former outperforms the latter in 60$\%$ cases, providing a comprehensive overview of their performance.
  %By introducing the acceptance and excellence line, we can conduct a relative and distributed evaluation (See Sec.~\ref{sec. evaluation metrics}).
  }
  \label{fig: intro}

\end{figure}



%as there are tons of degradation combinations in a large degradation space. 



% To analyze the bias of existing evaluation, we adopt the same process to generate 100 random real-DIV2K$\_$val sets from a large degradation model. 
% Fig.~\ref{fig: bsresr_cop} shows that \textbf{\textit{a single real test set will lead to completely opposite or indistinguishable comparison results.}} In addition, an averaging strategy is unsuitable to evaluate real-SR methods directly. The average PSNR difference on 100 random test sets is only 0.02dB in Fig.~\ref{fig: bsresr_cop}. The average score cannot reflect the overall performance and distribution information. Furthermore, if the goal is to improve the average score, we can simply push the performance of easy cases (e.g, small noise or blur), but at the expense of hard ones (e.g., complex degradation combinations). This will conflict with our primal goal. On the contrary, when we have obtained acceptable results on some easy cases, we should switch our attention to other hard ones to improve the overall performance. All these call for a new framework to comprehensively evaluate real-SR methods. 

% Directly testing on all degradations is obviously infeasible, as there are numerous degradation combinations in the vast degradation space. 

\textbf{How to generate test sets?} The above question involves another fundamental question: How to generate test sets? Existing works directly randomly apply a vast degradation space to a small test set (i.e., DIV2K\_val that includes 100 images) for the test set. Such an approach introduces two unstable factors. 1) Due to the vastness of the degradation space, randomly sampling 100 degradations is hardly representative of the entire degradation space. 2) To achieve stable performance, previous test sets apply a fixed degradation (e.g., bicubic with a fixed blur kernel) on the whole test set in classical and blind SR. However, real-SR applies a degradation in one image that  introduces uncertain bias. As shown in Fig.~\ref{fig: conventional performance}, evaluation comparisons on random test sets yield the opposite conclusion. Such observations also motivate us to design a more reasonable approach to benchmark existing real-SR methods.

\textbf{What is the objective of real-SR?} 

% calculate the average performance on a randomly-sampled small-sized test set based on an IQA metric (e.g., PSNR). However, we find that this evaluation protocol is fatally flawed. Due to the vastness of the degradation space, a small test set that is selected randomly cannot reliably represent the degradation space and may cause significant bias and randomness in the evaluation results, as illustrated in Fig.~\ref{fig: conventional performance}. In addition, the current evaluation metrics, such as PSNR and SSIM, are inadequate for assessing real-SR methods, as they typically average quantitative results across all testing samples, which may also lead to biased comparison results. For example, one method may outperform another on 60\% of the degradation types, but it may not achieve a higher mean PSNR value for the entire test set (Sec. \ref{sec: comparison with common protocol}). The average score cannot adequately represent the overall performance and distribution. 

% Furthermore, if the goal is to improve the average score, we could focus solely on enhancing the performance of simple cases (e.g., small noise or blur), which, however, would adversely affect difficult ones (e.g., complex degradation combinations). This would contradict our main objective. Instead, once we have achieved satisfactory outcomes in easy cases, we should divert our focus towards challenging ones to enhance the overall performance. The aforementioned points indicate the need for a new framework that can comprehensively evaluate the performance of real-SR methods.


%In addition, an averaging strategy is unsuitable to evaluate real-SR methods directly. The average PSNR difference on the two random test sets is only 0.025dB in Fig.~\ref{fig: conventional performance}. The average score cannot reflect the overall performance and distribution information. This strongly illustrates the previous evaluation would be significantly biased and thus cannot reflect the real performance of different real-SR methods.

% How to systematically evaluate the real-SR methods under
% such a large and complex degradation space is a very
% challenging issue. Fortunately, we observe that some degradations cause very similar visual results, as shown in
% Fig.~\ref{fig: similiarity}. This inspires us that we can represent the huge degradation space by using limited representative degradations. Based on the representation, we could exploit a systemic evaluation framework for real-SR methods. Fig.~\ref{fig: distributed performance} shows the distributed performance on the representative degradations. We find that BSRNet performs clearly better than RealESRNet in most degradation cases. On the contrary, the results in Fig.~\ref{fig: conventional performance} show the great randomness of the conventional protocol, so it may lead to biased judgments. The comparison demonstrates that our framework can evaluate real-SR models more clearly and comprehensively.

% To analyze the bias of existing evaluation, we adopt the same process to generate 100 random real-DIV2K$\_$val sets from a large degradation model. 
% Fig.~\ref{fig: bsresr_cop} shows that the maximum difference between BSRNet and RealESRNet is 0.18dB on 1st test dataset, and the minimum difference is -0.23dB on the 100-th test dataset. There also exists a difference close to 0 on the 60-th test set. This observation reveals that \textit{\textbf{current evaluation can not provide an accurate comparison on a single random test set.}} 
% In addition, the average PSNR difference on 100 random test sets is only 0.02dB in Fig.~\ref{fig: bsresr_cop} as different degradations may have different quantitative results. Therefore, the average performance is no longer sufficient for the needs of real-SR evaluation.


% In addition to the above dilemma, existing evaluation metrics (e.g., PSNR and SSIM) are also not suitable to directly evaluate real-SR methods. Specifically, they generally average quantitative results on all testing samples, but such an averaging strategy may also bring biased comparison results. For example, one method may surpass the other one on 60\% degradation types, but it may not get a higher mean PSNR value on the whole test set (Sec. \ref{sec: comparison with common protocol}). The average score cannot reflect the overall performance and distribution information. Furthermore, if the goal is to improve the average score, we can simply push the performance of easy cases (e.g, small noise or blur), but at the expense of hard ones (e.g., complex degradation combinations). This will conflict with our primal goal. On the contrary, when we have obtained acceptable results on some easy cases, we should switch our attention to other hard ones to improve the overall performance. All these call for a new framework to comprehensively evaluate real-SR methods. 

% In this paper, we propose a complete evaluation framework, including a degradation clustering method, acceptance and excellence lines, and a systematic evaluation protocol with new evaluation metrics, dedicated to real-SR methods. 


In this work, we establish a systematic evaluation framework that assesses relative, distributed, and overall performance rather than relying solely on absolute, average, and biased performance metrics commonly used in current evaluation methods. Our first step is to use a clustering approach to partition the expansive degradation space to identify representative degradations. Subsequently, we utilize these representative degradations to create a distributional test set. In the second step, we propose an evaluation protocol that incorporates two new relative evaluation metrics, namely Acceptance Ratio ($AR$) and Relative Performance Ratio ($RPR$), with the introduction of acceptance and excellence lines. The $AR$ metric indicates the percentage by which the real-SR method surpasses the acceptance line, which is a minimum quality benchmark required for the method to be considered satisfactory. The $RPR$ metric measures the improvement of the real-SR method relative to the distance between the acceptance and excellence lines. The integration of these metrics intends to provide a more refined and accurate evaluation of real-SR methods. With the proposed framework, it becomes possible to conduct a comprehensive evaluation of the overall performance of existing real-SR methods, as illustrated in Fig.~\ref{fig: distributed performance}.

The significance of this work can be summarized as:
\begin{itemize}
\item Our proposed evaluation framework is a first step towards a new paradigm for evaluating real-SR in a fair and comprehensive way.

\item Under the proposed evaluation framework, we benchmark existing real-SR methods and obtain new observations and valuable insights. Further, we employ the framework to develop a new strong baseline that achieves state-of-the-art overall performance. 

\item Our proposed evaluation framework has a general applicability that can facilitate the development of appropriate test sets and comparative evaluation metrics for real-SR.

%We propose a clustering-based evaluation framework to generate representative degradation cases, which are used to construct a group of test sets for real-SR evaluation on a large degradation space.
%\item We propose two new metrics -- Acceptance ratio ($AR$) and Relative performance ratio ($RPR$) to perform systematic evaluation of real-SR models by introducing acceptance and excellence line.
%\item We benchmark the existing real-SR methods to obtain new observations and insights. Then, we employ the proposed evaluation framework to develop a new strong baseline, which achieves SOTA performance.  

\end{itemize}

%Thirdly, we benchmark the existing real-SR methods, conduct a series of observations, and gain numerous valuable insights. 
%Finally, we use the proposed framework to explore the impact of basic strategies on the real-SR model and then use the optimal training strategies to introduce a simple yet powerful baseline, which achieves SOTA performance compared with the existing methods. 
%In this paper, we propose a systematic evaluation framework that measures relative, distributed, and overall performance instead of focusing on absolute, average, and biased performance as in existing methods.
%First, we use a spectral clustering approach to divide a large degradation space to find representative degradations. Then, we use the representative degradations to generate a distributional test set.
%Second, by introducing acceptance and excellence lines, we propose an evaluation protocol with two new relative evaluation metrics – Acceptance Ratio ($AR$) and Relative Performance Ratio ($RPR$). $AR$ denotes the percentage that the real-SR method is better than the acceptance line, while $RPR$ represents the relative improvement of the real-SR method compared with the distance between acceptance and excellence lines. 
%Thirdly, we benchmark the existing real-SR methods, conduct a series of observations, and gain numerous valuable insights. 
%Finally, we use the proposed framework to explore the impact of basic strategies on the real-SR model and then use the optimal training strategies to introduce a simple yet powerful baseline, which achieves SOTA performance compared with the existing methods. 
% To further provide a holistic view of model performance, we plot the distributions of their performance with the acceptance line (i.e., FSRCNN-mz) and excellent line (i.e., SRResNet-mz) in PSNR calculated on the 100 representative degradations in Fig.~\ref{fig: basis performance}. We can see that BSRNet performs clearly better than RealESRNet on most degradation cases. On the contrary, the results in Fig.~\ref{fig: bsresr_cop} show the great randomness of the conventional protocol, so it may lead to biased or unfair judgments. The comparison demonstrates that our protocol can evaluate real-SR models more clearly and comprehensively.

% In this paper, we propose a complete evaluation pipeline, including a degradation clustering method, acceptance and excellence lines, and a systematic evaluation protocol with new evaluation metrics, dedicated to real-SR methods. Different from traditional evaluation strategies, our method evaluates relative, distributed, and overall performance, instead of absolute, average, and biased performance. First, to evaluate the overall performance, we combine different degradation models to generate a large degradation space that could cover most real-world cases. Then, we adopt spectral clustering to divide this space into a hundred sub-spaces and use their cluster centers as representative degradation types. Second, to evaluate the relative and distributed performance, we propose acceptance and excellence lines as comparison baselines, which contain a series of SR networks trained with the degradation parameters of the cluster centers. We then introduce two new evaluation metrics – Acceptance Ratio ($AR$) and Relative Performance Ratio ($RPR$) to comprehensively evaluate the relative and distributed performance over a large degradation space. Finally, we propose a systematic evaluation protocol to benchmark the existing real-SR methods. As shown in Fig.~\ref{fig: intro}, $AR$ denotes the percentage that the real-SR method is better than the acceptance line, while $RPR$ represents the relative improvement of the real-SR method compared with the distance between acceptance and excellence lines. 

% We use the proposed protocol to explore the impact of basic strategies on the real-SR model and then use the optimal training strategies to introduce a simple yet powerful baseline, which achieves SOTA performance compared with the existing methods. 

% The contributions of this paper are summarized as follows:




